Star formation history of the solar neighbourhood as told by Gaia

The Gaia DR2 catalog is the best source of stellar astrometric and photometric data available today. The history of the Milky Way galaxy is written in stone in this data set. Parallaxes and photometry tell us where the stars are today, when were they formed, and with what chemical content, i.e. their star formation history (SFH). We develop a Bayesian hierarchical model suited to reconstruct the SFH of a resolved stellar population. We study the stars brighter than $G\,=\,15$ within 100 pc of the Sun in Gaia DR2 and derive a SFH of the solar neighbourhood in agreement with previous determinations and improving upon them because we detect chemical enrichment. Our results show a maximum of star formation activity about 10 Gyr ago, producing large numbers of stars with slightly below solar metallicity (Z=0.014), followed by a decrease in star formation up to a minimum level occurring around 8 Gyr ago. After a quiet period, star formation rises to a maximum at about 5 Gyr ago, forming stars of solar metallicity (Z=0.017). Finally, star formation has been decreasing until the present, forming stars of Z=0.03 at a residual level. We test the effects introduced in the inferred SFH by ignoring the presence of unresolved binary stars in the sample, reducing the apparent limiting magnitude, and modifying the stellar initial mass function.

==> A3_solar_neighbourhood.tex <==
\section{Modelling the Solar Neighbourhood}\label{snmod}
\input{table_C1}
\input{table_C2}
\input{figure_C1}
\input{figure_C2}

As a sanity check, we model the solar neighbourhood population using the values of $a_i$ derived above as input to the MW.mx Galaxy model described in Appendix\,\ref{mw.mx}. 
We interpret the populations detected in Section\,\ref{amd} as belonging to the {\it thin disc}.
We map each of the eleven components per $Z$ listed in the full version of Table\,\ref{tab:4} (available as supplementary online material) to one of the seven thin disc age groups used in MW.mx, defined in Table\,\ref{tab:B2}.
Table\,\ref{tab:C1} lists the resulting fractional weights $a^{*}_i$ for the percentiles $p10$, $p50$ (median) and $p90$. 
The number of stars with $G\leq15$ belonging to each group is then $a^{*}_i \times 120,452$ (cf. Section\,\ref{samp_sel_sol}).
We perform 10 Monte Carlo simulations of \solm\ for each set of $a^{*}_i$ in Table\,\ref{tab:C1} (\simn, hereafter) and another 10 simulations using the age groups as defined in the three rightmost columns of Table\,\ref{tab:B2} (\simm, hereafter).
In \simn\ the simulation is stopped when we reach the required number of stars with $G\leq15$ for each component, irrespective of the accumulated mass.
In contrast, in \simm\ the simulation is continued until we reach the total mass for each population, obtained by integration of $\rho(R,z)$ over the given volume, irrespective of the number of stars with $G\leq15$.
For more realistic results, we use the trends of the errors on $\varpi,\,G,\,G_{BP}$ and $G_{RP}$ determined from \gtwo
to add Gaussian noise to the parallax $\varpi^*$ and apparent $G^*,\,G^*_{BP}$ and $G^*_{RP}$ magnitudes of each star in the \simn\ and \simm\ simulations.

Fig.\,\ref{fig:8}, discussed in Section\,\ref{qc}, shows the average number counts in the $G$ band resulting from our simulations. 
Fig.\,\ref{fig:C1} shows the contribution to the number counts from each of the thin disk age groups. Stars younger than 2 Gyr (groups 1, 2, 3) account for 85\% of the stars brighter than $G=6$ in \simm\ but only for 55\% of these stars in \simn. Group 7 contributes about 50\% of the stars fainter than $G=8$ in \simn, but no group contributes more than 20\% in \simm. In Table\,\ref{tab:C2} we list relevant astrophysical properties of the solar neighbourhood derived from these simulations. The stellar population of \sols\ is more numerous, less massive, and brighter according to \simm\ than to \simn, resulting in a lower $M/L$ ratio in the \simm\ simulation. This is consistent with the brightness profile in Fig.\,\ref{fig:C1} which shows that the integrated magnitude of \sols\ is 1 magnitude brighter in \simm\ than in \simn. Observations at the bright end of the same quality as {\it Gaia}'s are needed to judge in favour or against one of these scenarios.

% Fig.\,\ref{fig:8} shows the average number counts in the $G$ band resulting from our simulations.
% The agreement of the counts for both sets of simulations in the range $G=[8,18]$ is remarkable given the differences in the models and 
% may indicate the lack of sensitivity of the number counts to the model ingredients.
% The reasons for the excess counts at the bright end in the simulations with respect to \gtwo\ have been analyzed in Section\,\ref{samp_sel_sol}.
% The \gtwo\ counts are clearly complete to $G=15$.
% By construction, the \simn\ simulation follows more closely the observed number counts than the \simm\ simulation.
% Since at the bright end the observed counts are underestimated, it is interesting to explore the nature of the brighter stars in the simulations.
% Fig.\,\ref{fig:C1} shows the contribution to the number counts from each of the thin disk age groups.
% Stars younger than 2 Gyr (groups 1, 2, 3) account for 85\% of the stars brighter than $G=6$ in \simm\ but only for 55\% of these stars in \simn.
% Group 7 contributes about 50\% of the stars fainter than $G=8$ in \simn, but no group contributes more than 20\% in \simm.
% In Table\,\ref{tab:C2} we list relevant astrophysical properties of the solar neighbourhood derived from these simulations.
% The stellar population of \sols\ is more numerous, less massive, and brighter according to \simm\ than to \simn, resulting in a lower $M/L$ ratio in the \simm\ simulation.
% This is consistent with the brightness profile in Fig.\,\ref{fig:C1} which shows that the integrated magnitude of \sols\ is 1 magnitude brighter in \simm\ than in \simn.
% Observations at the bright end of the same quality as {\it Gaia}'s are needed to judge in favour or against one of these scenarios.
% 
% In Fig.\,\ref{fig:9} we compare the \gtwo CMD of \solm\ with \simn\ and \simm. 
% The rightmost panel in the {\it top} and {\it middle rows} show the residuals \simn\,-\,\solm\ and \simm\,-\,\solm, respectively, colour coded as indicated in the auxiliary axis.
% The residuals show a deficit of stars on the red side of the MS, and an excess on the blue side.
% The positive residual is more marked and extends to brighter magnitudes in \simm\ than in \simn.
% Similar residual CMD's are presented in \citet[][their figure 1]{Mor19}.
% We think that the behavior of the residuals in Fig.\,\ref{fig:9} is due to the fact that in our derivation of the vector $\bm{a}$ we do not correct for the presence of unresolved binary stars in the \solm sample. As illustrated in Section\,\ref{ub}, unresolved binary systems broaden the locus defined by single star isochrones in the CMD. An unresolved companion makes a MS primary star look {\it redder, brighter and more massive} in the CMD than it really is. It is then natural that our Bayesian inference lacks stars that are near the MS but redder than in the single star isochrones used as priors. When the primary star is a WD the unresolved system may appear bluer (Section\,\ref{ub}) but these systems are less frequent. In the {\it bottom row} of Fig.\,\ref{fig:9} we show the observed and simulated (\simn) CMDs of \solm.
% The {\it red dots} in the rightmost panel indicate the expected position of unresolved binary systems for a 1 Gyr, $Z=0.014$ population.
% When the binary population is added to all the isochrones entering our model, the red strip in this panel becomes broader.

For completeness, in Fig.\,\ref{fig:C2} ({\it top row}) we compare the CMDs resulting from the \simn\ and \simm\ simulations. 
The residuals \simn\,-\,\simm\ show an excess of stars on the red side of the MS and a deficit on the blue side. 
In the {\it bottom row} we compare two \simn\ simulations to illustrate the flat residuals expected when comparing unbiased samples. 
Even though in \simn\ there are not enough stars on the red side of the single star MS to explain the observations, there are more of these stars in \simn\ than in \simm.
Figs.\,\ref{fig:9} and \ref{fig:C2} show CMDs for simulations computed with the $p50$ values of $a^{*}_i$ in Table\,\ref{tab:C1}.
CMDs for $p10$ and $p90$ are available as supplementary online material (Figs.\,14,\,15, and 16). 

The net effect of unresolved binaries is then to widen the single star MS in the CMD towards both {\it brighter-and-redder} and {\it fainter-and-bluer} magnitudes.
This may explain the width of the MS in the \gtwo CMD of Figs.\,\ref{fig:1} and \ref{fig:9}.
As pointed out by \cite{kr01}, the single-star IMF may also be steeper than inferred from observations that do not resolve binary systems. 
The biases introduced by unresolved binaries in the determination of the SFH using our statistical model will be the subject of a future paper.


==> figure_12e.tex <==
\begin{figure}
\begin{center}
    \includegraphics[width=1.12\columnwidth]{FIGURES/alzate_et_al_figure_12e.png}
    \caption{\label{fig:12e}Distribution of {\it absolute} $M_G$ magnitude for all the stars in the 
    \sola\ (47,799 stars),
    \solb\ (63,686 stars),
    \solc\ (86,516 stars), and
    \solm\ (120,452 stars) sub-samples.}
\end{center}
\end{figure}
% \textcolor{blue}{Star numbers S12, S13, S14, S15 = S15: 120452 S14: 86516 S13: 63686 S12: 47799}


==> figure_16.tex <==
\begin{figure*}
\begin{center}
   \includegraphics[width=\textwidth]{FIGURES/alzate_et_al_figure_16a.pdf}
   \includegraphics[width=\textwidth]{FIGURES/alzate_et_al_figure_16b.pdf}
   \includegraphics[width=\textwidth]{FIGURES/alzate_et_al_figure_16c.pdf}
   \includegraphics[width=\textwidth]{FIGURES/alzate_et_al_figure_16d.pdf}
   \caption{\label{fig:16}AMD for the \solm\ sample inferred assuming
      {\it (a)} the \citet{salp55},
      {\it (b)} the \citet{kr01}, 
      {\it (c)} the case A \citet{Mor19} and
      {\it (d)} the case B \citet{Mor19} IMF, the grid C of isochrones listed in Table\,\ref{tab:4} with no extinction correction, and $\sigma_{i}$\,=\,0.075.
      The height of the bars in the 3D plots on the left hand side is the median of the distribution of $a_i$ for the corresponding isochrone.
      The violin plots summarize the marginalized {\it posterior} PDF for age and $Z$.
      The horizontal lines in each violin represent from bottom to top the 0, 50, and 100 percentiles of the distribution.
      The figure in panel {\it (b)} duplicates Fig.\,\ref{fig:6}c with a different vertical scale.}
\end{center}
\end{figure*}


==> table_C2b.tex <==
% \begin{table*}
% \caption{\label{tab:C2}Global properties of the solar neighbourhood stellar population.
% $N_{*}$, $M_{*}$ and {\bf G}$_{*}$ are, respectively, the number, total mass and integrated absolute $G$ magnitude of the stars
% in the simulation brighter than the limiting magnitude. $M/L_G$ was computed using $G_\odot=5$.}
% \begin{tabular}{lrrrrrrrrrrrr}
% \hline
% Simulation:        & \mc{3}{c}{Sim N} &&& \mc{3}{c}{Sim N} &&& \mc{2}{c}{Sim M} \\
% Limiting magnitude & \mc{3}{c}{$G \leq 15$} &&& \mc{3}{c}{$G \leq 20$} &&& \mc{1}{c}{$G \leq 15$} & \mc{1}{c}{$G \leq 20$} \\
% \hline
% Percentile & \mc{1}{c}{p50} & \mc{1}{c}{p10} & \mc{1}{c}{p90} &&& \mc{1}{c}{p50} & \mc{1}{c}{p10} & \mc{1}{c}{p90} \\
% $N_{*}$                           & 120551   &  70633 & 191900 &&&   358037 & 210225 &   568974 &&&  126405 &    341223 \\
% $M_{*}$ (M$_\odot$)               &  76443   &  44111 & 122933 &&&   159810 &  93553 &   255398 &&&   84597 &    151613 \\
% {\bf G}$_{*}$                     &  -7.97   &  -7.22 &  -8.59 &&&    -7.97 &  -7.22 &    -8.59 &&&   -8.77 &     -8.77 \\
% $M/L_{G}$    (M$_\odot/L_{\odot}$)&   0.49   &   0.57 &   0.45 &&&     1.03 &   1.22 &     0.94 &&&    0.26 &      0.47 \\
% \hline
% \end{tabular}
% \end{table*}

\begin{table}
\caption{\label{tab:C2}Global properties of the solar neighbourhood stellar population.
$N_{*}$, $M_{*}$ and {\bf G}$_{*}$ are, respectively, the number, total mass and integrated absolute $G$ magnitude of the stars
in the simulation brighter than the limiting magnitude. $M/L_G$ was computed using $G_\odot=5$.}
\begin{tabular}{lrrr}
\hline
Simulation:        & \mc{3}{c}{Sim N}                                               \\ %&&& \mc{3}{c}{Sim N} &&& \mc{2}{c}{Sim M} \\
Limiting magnitude & \mc{3}{c}{$G \leq 15$}                                         \\ %&&& \mc{3}{c}{$G \leq 20$} &&& \mc{1}{c}{$G \leq 15$} & \mc{1}{c}{$G \leq 20$} \\
\hline
Percentile & \mc{1}{c}{p50} & \mc{1}{c}{p10} & \mc{1}{c}{p90}                       \\ % &&& \mc{1}{c}{p50} & \mc{1}{c}{p10} & \mc{1}{c}{p90} \\
$N_{*}$                           & 120551   &  70633 & 191900                       \\ % &&&   358037 & 210225 &   568974 &&&  126405 &    341223 \\
$M_{*}$ (M$_\odot$)               &  76443   &  44111 & 122933                       \\ % &&&   159810 &  93553 &   255398 &&&   84597 &    151613 \\
{\bf G}$_{*}$                     &  -7.97   &  -7.22 &  -8.59                       \\ % &&&    -7.97 &  -7.22 &    -8.59 &&&   -8.77 &     -8.77 \\
$M/L_{G}$    (M$_\odot/L_{\odot}$)&   0.49   &   0.57 &   0.45                       \\ % &&&     1.03 &   1.22 &     0.94 &&&    0.26 &      0.47 \\
\hline
\\
\hline
Simulation:        & \mc{3}{c}{Sim N}                                               \\ %&&& \mc{3}{c}{Sim N} &&& \mc{2}{c}{Sim M} \\
Limiting magnitude & \mc{3}{c}{$G \leq 20$}                                         \\ %&&& \mc{3}{c}{$G \leq 20$} &&& \mc{1}{c}{$G \leq 15$} & \mc{1}{c}{$G \leq 20$} \\
\hline
Percentile & \mc{1}{c}{p50} & \mc{1}{c}{p10} & \mc{1}{c}{p90}                       \\ % &&& \mc{1}{c}{p50} & \mc{1}{c}{p10} & \mc{1}{c}{p90} \\
$N_{*}$                           &  358037 & 210225 &   568974                     \\ % &&&  126405 &    341223 \\
$M_{*}$ (M$_\odot$)               &  159810 &  93553 &   255398                     \\ % &&&   84597 &    151613 \\
{\bf G}$_{*}$                     &   -7.97 &  -7.22 &    -8.59                     \\ % &&&   -8.77 &     -8.77 \\
$M/L_{G}$    (M$_\odot/L_{\odot}$)&    1.03 &   1.22 &     0.94                     \\ % &&&    0.26 &      0.47 \\
\hline
\\
\hline
Simulation:        & \mc{2}{c}{Sim M}                                           &  \\ 
Limiting magnitude & \mc{1}{c}{$G \leq 15$} & \mc{1}{c}{$G \leq 20$}            &  \\
\hline
$N_{*}$                           &  126405 &    341223                         & \\
$M_{*}$ (M$_\odot$)               &   84597 &    151613                         &  \\
{\bf G}$_{*}$                     &   -8.77 &     -8.77                         &  \\
$M/L_{G}$    (M$_\odot/L_{\odot}$)&    0.26 &      0.47                         &  \\
\hline
\end{tabular}
\end{table}

